ProNet: Network-level Bandwidth Sharing among Tenants in Cloud

In today's private cloud, the resource of the datacenter is shared by multiple tenants. Unlike the storage and computing resources, it's challenging to allocate bandwidth resources among tenants in private datacenter networks. State-of-the-art approaches are not effective or practical enough to meet tenants' bandwidth requirements. In this paper, we propose ProNet, a practical end-host-based solution for bandwidth sharing among tenants to meet their various demands. The key idea of ProNet is byte-counter, a mechanism to collect the bandwidth usage of tenants on end-hosts to guide the adjustment of the whole network allocation, without putting much pressure on switches. We evaluate ProNet both in our testbed and large-scale simulations. Results show that ProNet can support multiple allocation policies such as network proportionality and minimum bandwidth guarantee. Accordingly, the application-level performance is improved.

==> eurosys/sections/algorithm-design.tex <==
\section{Alogorithm design}
\label{sec5}

One of the challengest problems of our system development is the design of the allocation algorithms. Our designed algorithms should be flexible enough to suit the changeable data center environment and react fastly also with relatively low workloads for all parts of the system in the data center.

Here we basically present four algorithms that can represent the main ideas of our system design. 

\subsection{Bandwidth Functions Transformation Algorithm}
This function is implied for the aggregation of the \textbf{bandwidth function}s, which is used in the \textbf{Rate Control Layer} for the aggregation of the function of tenants and its unit-flows'. This function is mainly based on the Hierarchical MPFA algorithm from the \sys~ paper[], and we have modified it for the adaption of the tenants' preference features into a \textbf{bandwidth function} in the \textbf{Rate Control Layer}. 

The initial \textbf{bandwidth function} we usually choose for each unit-flow is:

\begin{equation}\label{1}
B_x(s)=\min{\left(srcWeight+dstWeight,\ deviceRateLimit\right)} 
\end{equation}

In \eqref{1}, $srcWeight$ is the weight of the source host’s weight and the $dstWeight$ is the weight of the destination host’s weight, as the $deviceRateLimit$, is the rate limitation of that host. By using this initial function, we are able to add the information of the preference to each host for every tenant.

Because a \textbf{bandwidth function} is usually a sectionally continuous function, so that we can represent a \textbf{bandwidth function} as a group of interesting points (the points that slop of function is zero) of the function in convenience. The main goal \textbf{bandwidth function} $B_A^e\left(s\right)$ must satisfy this equation:

\begin{equation}\label{2}
\forall s,\ \sum_{\forall i|i\epsilon A}{B_i\left(s\right)=}B_A^e\left(s\right)
\end{equation}

For the aggregation state, firstly, for each tenants A, we create a add up \textbf{bandwidth function} for all its unit-flows:

\begin{equation}\label{3}
\forall s,\ B_A^a\left(s\right)=\ \sum_{\forall i\epsilon A} B_i\left(s\right)
\end{equation}

Then calculate a function $T_A$ which we call it transforming function about \textit{fair share} from $B_A^a\left(s\right)$ to $B_A\left(s\right)$:

\begin{equation}\label{4}
T_A\left(s\right)=\ \bar{s}|B_A^a\left(s\right)=\ B_A\left(\bar{s}\right)
\end{equation}

For each $x\in A$, apply $T_A$ on $B_A$'s  \textit{fair share} to get $B_A^e$:

\begin{equation}\label{5}
B_A^e\left(T_A\left(s\right)\right)=B_A\left(s\right)
\end{equation}

In this way, we can get an aggregation \textbf{bandwidth function} which can both satisfy the condition of the \textbf{bandwidth function} of the tenant itself and the restriction of each unit-flow it contains.

\subsection{Target Status Estimation Algorithm}
This is a simple algorithm used in the \textbf{Bandwidth-coordinator} to calculate the next step's new allocation target when the coordinator every time collects all the tenants'allocation information and all the usage from the lower level from the last time cycle, then calculates the new fair share used by all the tenants.

In the below expresions, $s_i$ is the \textit{fair share} from tenants at $i$ in that time.
The input of this is function is an array containing all the collected \textit{fair share} from each tenant.
Firstly, calculate the average value of all the \textit{fair share}:

\begin{gather}
InputArray=[s_1,\ s_2,\ s_3,\ \ldots,\ s_N]\label{6}\\
Avg=average(InputArray)\label{7}
\end{gather}

Due to many situations, those \textit{fair share}s might not be equal (means unfairly allocation might happen in the last time cycle). Therefore, we should adjust the \textit{fair share} for the next allocation cycle. Also, we add an accelerated session in this function, $alpha$ is a growth parameter:

\begin{gather}
Diff\ =\ InputArray-[Avg,\ Avg,\ Avg,\ \ldots,\ Avg]\label{8}\\
Target\ =\ Avg\ \ast\ \left(1\ +\ alpha\right)\label{9}\\
OutputArray\ =\ [Target,\ Target,\ \ldots,\ Target]-Diff\label{10}
\end{gather}

After this, the \textbf{Bandwidth-coordinator}  will send the new \textit{fair share}s which is in OutputArray to all the \textbf{Rate-controllers} for the further jobs.


\subsection{Distributed Edge Optimization Algorithm}
This is an algorithm that functions in every \textbf{Rate-Controler} when they receive the new targets from \textbf{Bandwidth-coordinator}. By using this algorithm, our system can achieve distributedly optimize the bandwidth allocation in each host. We set a variable $rateSum$ which represents the bandwidth usage of this host and $deviceRateLimit$ stands for the Rate limit of this host and a learning rate $k$. We also use $scalingFactor$ to handle the situation when is over-allocated here. A lower bound of fair share is set here as $LShare$. Also if a host receives CAWC feedback from the receiving host, the optimization behavior will change due to some of the tenants' flow having reached a congested condition and the rate of the sending host should be controlled.

\begin{algorithm}\footnotesize
\caption{Distributed Edge Optimization Algorithm} 
\hspace*{0.02in} {\bf Input:} 
$GlobalTargetFairShare$\\
\hspace*{0.02in} {\bf Output:} 
The allocation result rate for each unit-flow
\begin{algorithmic}[1]
\State This algorithm periodly runs at the $rateControlCycle$ 
\For{$flow$ in $flowTable$} 
	\If{flow's $BandwidthUsage==0$} 
	\State flow's FairShare = $0$
	\State flow's ExpairedFlag = $1$
	\EndIf
	\If{flow's ExpairedFlag==0}
	\State $oldFS=max(flow's Fair Share, minValue)$
	\If{flow's CongestionFactor>=$CongestionThreshold$ or $deviceRateLimitFlag$ is true}
	\State $newFS=oldFS+(GlobalTargetFairShare - oldFS)*k$
	\ElsIf{flow's BandwidthUsage!=0}
	\State $newFS=oldFS*(1+rateControlCycle/reportCycle)$
	\EndIf
	\State flow's FairShare = $newFS$
	\State $rateSum+=flow's BandwidthUsage$
	\EndIf
\EndFor
\If{$rateSum==0$}
\State $rateSum = deviceRateLimit * 0.1$
\EndIf
\If{$rateSum >= deviceRateLimit$}
\State  $scalingFactor *= (deviceRateLimit / rateSum)$
\State $deviceRateLimitFlag = true$
\Else 
\State $deviceRateLimitFlag = false$ 
\EndIf
\State $rate = rateSum * scalingFactor$
\For{$flow$ in $flowTable$}
\State $flow's\ rate=flow's\ rate *scalingFactor$
\EndFor
\end{algorithmic}
\end{algorithm}

In this algorithm, for each unit-flow on the flow table, which is maintained by each \textbf{Rate-contoller} on each host, with a set time cycle. When the \textbf{Rate-contoller} receives the new \textit{TargetFairShare} from the \textbf{Rate-coordinator}, it will distributedly optimize the next allocation goal for each unit-flow. There are many conditions. For instance, the unit-flows that are in congestion conditions will be rate-limited and scaled for the performance. As for the unit-flows not in congestion state and in the working state will be enforced for rate accelerate to achieve work-conserving. 

After all this work, we can achieve a fairly bandwidth-distributed allocation among tenants in a short convergence time.
\subsection{CAWC Algorithm}
This is the Congestion-Aware Work-Conserving mechanism, which we make for congestion detection inside the network. The basic idea of this algorithm is to use the ECN mechanism. Each host in our design maintains a scoreboard, and the scoreboard will count the receiving packets' types and record the bytes number of them. On the scoreboard, we keep counting the number of normal packets' bytes and the bytes of the packets' with ECN tags on. By using this data, we keep a sliding window depending on the congestion degree inside the network. According to the Volume of the sliding window, with the counter of the bytes in the ratio of the packets with ECN tags, the receiving host will thus decide whether to send the special feedback packet as the congestion signal to the sending host or not. This kind of packet is set as the top priority in our system to guarantee control quality.



==> eurosys/sections/system-design.tex <==
\section{System Design}
\label{sec4}

\begin{figure}
	\centering
	\setlength{\abovecaptionskip}{0 cm}
	\includegraphics[width=3.5in]{figures/fig2.png}
	\caption{System Structure}
\end{figure}


In this paper, we focus on the overall bandwidth allocation inside the data center among tenants. Figure 2 shows the basic framework of \sys~. It is shown that our system is designed hierarchically, there are two parts in our design: the lower \textbf{Traffic controller} and the upper \textbf{Rate Controller}. Traffic controller is the place where we actually control the network traffic of the sending end to enforce the allocation fairness goal of bandwidth. As for the Rate controller, this is the stage where our allocation algorithms and strategies show off. Rate controller will get the usage from each unit-flow' s bytes-counter in the set time cycle. After the process of our algorithms, the Rate Controller then will send the new command to each unit-flow for the next step allocation. Also, the Rate Controller will get the ECN message from the receiving host as input of our CAWC mechanism. In this way we can ensure the congestion will not happen in the sending port to avoid unnecessary packets dropping.

\subsection{Traffic Controller}
Traffic controller is the place that deals with the actual network flows.

\noindent\textbf{Network Slicing: }In the process of the Traffic Controller, what we do first is to handle the flows ready to be sent in the sending queue. What we do here is slicing the flows. For packets in the sending queue, Traffic controller will regroup them into different unit-flows. For the packets in each unit-flow, they have the same source and destination address and belong to the flow of the same tenant.
%When the sending flow of the host generates and prepares to be sent, they will be processed firstly by the Flow-slider. The function of the slider is to cut the network flows into unit-flows, which decide on the address information and which tenant the packets of the flow belong to.

\noindent\textbf{Rate limiting: }After that, the task of this Traffic controller later is basically to receive the command from the Rate Controller and rapidly adjust the rate of each unit-flow. After several evaluations and tests we made, we choose to use Token Bucket Filter (TBF)[] as the rate limiter of each unit-flow. The token bucket algorithm is based on an analogy of a fixed capacity bucket into which tokens, which represent a unit of bytes, are added at a fixed rate, which is the average set rate. When a packet is to be checked for conformance to the defined limits, the bucket is inspected to see if it contains sufficient tokens at that time. If so, the equivalent number of tokens to the length of the packet in bytes is removed, and the packet is sent. The packet does not confirm if there are insufficient tokens in the bucket, and the contents of the bucket are not changed. The reason we use TBF is that it can provide relative average rate control, also with the second bucket of TBF, the peak rate of TBF is controllable, which is an essential guarantee in rate control. In our design, we have assigned a TBF to each unit-flow for rate management.In this way, our system can manage each tenants' flow isolately. 

\noindent\textbf{Allocation behavior initiation: }Also, for each unit-flow, a bandwidth function is attached to it, which is stored inside the Rate Controller and represents the allocation plan of this simple unit. Of course, we can't manually set all functions of each unit-flows, so they are automatically initialized according to the convergence time and the initial bandwidth we want for the flows. Normally, the initial bandwidth function is depending on the source and destination hosts' weight and the device (host)s' rate limits which is:

\begin{equation}\label{1}
B_x(s)=\min{\left(srcWeight+dstWeight,\ deviceRateLimit\right)} 
\end{equation}

In \eqref{1}, $srcWeight$ is the weight of the source host’s weight and the $dstWeight$ is the weight of the destination host’s weight, as the $deviceRateLimit$, is the rate limitation of that host. By using this initial function, we are able to add the information of the preference to each host for every tenant. Sometimes a tenant may even have preferences for each host. For example, one tenant may want one host to send twice as much as others, and this also can be achieved by setting the bandwidth function of each unit-flows when initialized. 

A bytes-counter is also installed at each unit-flow for the statistic of network usage. After this, the Rate Controller will periodically collect the usage from each unit-flow by the group of tenants and send back the new rate to be limited after the calculation. After receiving the newly assigned rate, the TBF from each unit-flow will then determine that rate.

\begin{figure}
	\centering
	\setlength{\abovecaptionskip}{0cm}
	\includegraphics[width=3.5in]{figures/fig3.png}
	\caption{Rate Controller Structure}
\end{figure}

\subsection{Rate Controller}
Rate Controller is where we actually apply our algorithm and control all the allocation among the whole system. Figure 3 shows the architecture of Rate controller. We can see that the Rate Controller is also a hieratical structure.

\noindent\textbf{Tenant-Controller: }This is the manager of each tenant, firstly will be assigned the preset bandwidth function which is able to reflect the allocation policy of that tenant. With each time cycle, the Tenant-Controller will collect all the usage and bandwidth function from each unit-flow that belongs to this tenant, and then aggregated all of the bandwidth functions into one simple bandwidth function, after that, the Tenant-controller will aggregate this function with the tenant itself's bandwidth function. Therefore, the all-new bandwidth function will contain all the allocation information from all unit-flows and the tenant itself. That's the way how we keep the allocation of one single tenant. In this way, if we can guarantee all of the tenants' unit-flow can be assigned with the correct bandwidth function, the fairness allocation in bandwidth will achieve naturally in our system. Next, we will explain the aggregation process.

\noindent\textbf{Tenants Bandwidth Function Aggregation Algorithm: }This function is implied for the aggregation of the BFs, which is used in the Rate Controller for the aggregation of the function of tenants and its unit-flows'. This function is mainly based on the Hierarchical MPFA algorithm from the BwE paper[], and we have modified it for the adaption of the tenants' preference features into a BF in the Rate Controller. 

Because a BF is usually a sectionally continuous function, so that we can represent a BF as a group of interesting points (the points that slop of function is zero) of the function in convenience. The main goal bf $B_A^e\left(s\right)$ must satisfy this equation:

\begin{equation}\label{2}
\forall s,\ \sum_{\forall i|i\epsilon A}{B_i\left(s\right)=}B_A^e\left(s\right)
\end{equation}

For the aggregation state, firstly, for each tenants A, we create a add up BF for all its unit-flows:

\begin{equation}\label{3}
\forall s,\ B_A^a\left(s\right)=\ \sum_{\forall i\epsilon A} B_i\left(s\right)
\end{equation}

Then calculate a function $T_A$ which we call it transforming function about \textit{fair share} from $B_A^a\left(s\right)$ to $B_A\left(s\right)$:

\begin{equation}\label{4}
T_A\left(s\right)=\ \bar{s}|B_A^a\left(s\right)=\ B_A\left(\bar{s}\right)
\end{equation}

For each $x\in A$, apply $T_A$ on $B_A$'s  \textit{fair share} to get $B_A^e$:

\begin{equation}\label{5}
B_A^e\left(T_A\left(s\right)\right)=B_A\left(s\right)
\end{equation}

In this way, we can get an aggregation bf which can both satisfy the condition of the BF of the tenant itself and the restriction of each unit-flow it contains.





\noindent\textbf{Allocation target planning: }With the usage report from each tenants' unit-flows, we can add up all of them to get the summary of the instance bandwidth usage from that tenant. Due to the linear increment characteristic of the bandwidth function, with the add up bandwidth usage, we can do reverse to get the right now fair shares of this tenant. For each host, the fair share of every tenant will be kept equal all the time for fairness. For high utilization, also each host's fair share will be accelerated.

\noindent\textbf{Bandwidth-coordinator: }However, there are many hosts inside the data center, and we can't only operate one single host. Instead, we must coordinate all of them to achieve overall fairness. For this purpose, we design the Bandwidth-coordinator. The job of this module is to arrange all the usage from each tenant for the statistical result from the last cycle and calculate and balance the fair share of each tenant below. The Bandwidth-coordinator will collect the last period's usage of each tenant and host to adjust the fair share of each host and tenant for the next period of time to keep the overall fairness in fair share and bandwidth allocation guarantee. After all the process, each new calculated fair share will be sent back to every tenant for the next round allocation. Next we will show how it works inside the Bandwidth-coordinator.

\noindent\textbf{Target Status Estimation Algorithm: }
This is a simple algorithm used in the Bandwidth-coordinator to calculate the next step's new allocation target when the coordinator every time collects all the tenants' allocation information and all the usage from the lower level from the last time cycle, then calculates the new fair share used by all the tenants.

In the below expresions, $s_i$ is the \textit{fair share} from tenants at $i$ in that time.
The input of this is function is an array containing all the collected \textit{fair share} from each tenant.
Firstly, calculate the average value of all the \textit{fair share}:

\begin{gather}
InputArray=[s_1,\ s_2,\ s_3,\ \ldots,\ s_N]\label{6}\\
Avg=average(InputArray)\label{7}
\end{gather}

Due to many situations, those \textit{fair share}s might not be equal (means unfairly allocation might happen in the last time cycle). Therefore, we should adjust the \textit{fair share} for the next allocation cycle. Also, we add an accelerated session in this function, $alpha$ is a growth parameter:

\begin{gather}
Diff\ =\ InputArray-[Avg,\ Avg,\ Avg,\ \ldots,\ Avg]\label{8}\\
Target\ =\ Avg\ \ast\ \left(1\ +\ alpha\right)\label{9}\\
OutputArray\ =\ [Target,\ Target,\ \ldots,\ Target]-Diff\label{10}
\end{gather}

After this, the Bandwidth-coordinator  will send the new \textit{fair share}s which is in OutputArray to all the Rate-controllers for the further jobs.




\noindent\textbf{Local Rate Optimization: }After each host receiving the new target fair share from the Bandwidth-coordinator, and then it will calculate new rate on demand for each unit-flow using the bandwidth function of it and it will be sent to the TBF for the new rate-limiting job. In this process, the hosts are not just simply calculating the target rates of unit-flows with the BF and the received fair share, instead the condition inside each host is different and complex. There are many other circumstances to consider such as the congestion inside the network or the expiration of some unit-flows. For the congestion inside the network, if it is detected, the growth rate of some tenants' unit-flows is suppose to be slow down. At the main time, to keep the allocation fairness, the rate of other tenants' unit-flows are also required to be adjusted. So the first problem is how can we aware the congestion inside network only with ProNet installed at the host ends? 

\noindent\textbf{CAWC Mechanism: }An important design in ProNet is what we call the Congestion-Aware Work-Conserving mechanism (CAWC). This is is designed for congestion detection inside the data center network among tenants. The basic idea of this algorithm is to use the ECN mechanism. Each host in our design maintains a scoreboard, and the scoreboard will count the receiving packets' types and record the bytes number of them. On the scoreboard, we keep counting the number of normal packets' bytes and the bytes of the packets' with ECN tags on. By using this data, we keep a sliding window depending on the congestion degree inside the network. According to the Volume of the sliding window, with the counter of the bytes in the ratio of the packets with ECN tags, the receiving host will thus decide whether to send the special feedback packet as the congestion signal to the sending host or not. This kind of packet is set as the top priority in our system to guarantee control quality. By using CAWC, the sending host-end will now easily be aware of the congestion situation caused by the flows that sent by the host itself and to get control of them.

Next the Rate Controller is going to do is summarize both the information come from the Bandwidth Coordinator and the CAWC feedback. Another algorithm is designed by us in this part. 

\noindent\textbf{Distributed Edge Optimization Algorithm: }This is an algorithm that functions in every Rate-Controller when they receive the new targets from Bandwidth-coordinator. By using this algorithm, our system can achieve distributedly optimize the bandwidth allocation in each host. We set a variable $rateSum$ which represents the bandwidth usage of this host and $deviceRateLimit$ stands for the Rate limit of this host and a learning rate $k$. We also use $scalingFactor$ to handle the situation when is over-allocated here. A lower bound of fair share is set here as $LShare$. Also if a host receives CAWC feedback from the receiving host, the optimization behavior will change due to some of the tenants' flow having reached a congested condition and the rate of the sending host should be controlled.

\begin{algorithm}\footnotesize
\caption{Distributed Edge Optimization Algorithm} 
\hspace*{0.02in} {\bf Input:} 
$GlobalTargetFairShare$\\
\hspace*{0.02in} {\bf Output:} 
The allocation result rate for each unit-flow
\begin{algorithmic}[1]
\State This algorithm periodly runs at the $rateControlCycle$ 
\For{$flow$ in $flowTable$} 
	\If{flow's $BandwidthUsage==0$} 
	\State flow's FairShare = $0$
	\State flow's ExpairedFlag = $1$
	\EndIf
	\If{flow's ExpairedFlag==0}
	\State $oldFS=max(flow's Fair Share, minValue)$
	\If{flow's CongestionFactor>=$CongestionThreshold$ or $deviceRateLimitFlag$ is true}
	\State $newFS=oldFS+(GlobalTargetFairShare - oldFS)*k$
	\ElsIf{flow's BandwidthUsage!=0}
	\State $newFS=oldFS*(1+rateControlCycle/reportCycle)$
	\EndIf
	\State flow's FairShare = $newFS$
	\State $rateSum+=flow's BandwidthUsage$
	\EndIf
\EndFor
\If{$rateSum==0$}
\State $rateSum = deviceRateLimit * 0.1$
\EndIf
\If{$rateSum >= deviceRateLimit$}
\State  $scalingFactor *= (deviceRateLimit / rateSum)$
\State $deviceRateLimitFlag = true$
\Else 
\State $deviceRateLimitFlag = false$ 
\EndIf
\State $rate = rateSum * scalingFactor$
\For{$flow$ in $flowTable$}
\State $flow's\ rate=flow's\ rate *scalingFactor$
\EndFor
\end{algorithmic}
\end{algorithm}

In this algorithm, for each unit-flow on the flow table, which is maintained by each Rate-controller on each host, with a set time cycle. When the Rate-controller receives the new \textit{TargetFairShare} from the Rate-coordinator, it will distributedly optimize the next allocation goal for each unit-flow. There are many conditions. For instance, the unit-flows that are in congestion conditions will be rate-limited and scaled for the performance. As for the unit-flows not in congestion state and in the working state will be enforced for rate accelerate to achieve work-conserving. 

And so on and so forth with a set time cycle, this sending host will achieve the convergence statute in a short time.

% An important design in \sys~ is what we call the Congestion-Aware Work-Conserving mechanism (CAWC). CAWC is designed for congestion detection inside the data center network among tenants. We use the Explicit Congestion Notification (ECN), which is a simple function supported by the nowadays commercial Switches to imply CAWC. CAWC can use the ECN tags in receiving packets and with the algorithms in it to calculate the congestion occurring place and what tenants' flows cause the congestion. With all this information, the receiving host will send our specific congestion signal back to the sending end. Then the sending end will adjust the growth rate of the sending rate of the corresponding unit-flows belonging to the congested tenants, and all of these adjustments are made with the allocation fairness as the premise.






%\begin{figure}
%  \centering
%  \subfigure[Intra-tenant Congestion]{\includegraphics[width=1.5in]{figures/fig4(a).png}}
%  \subfigure[Inter-tenants Congestion]{\includegraphics[width=1.5in]{figures/fig4(b).png}}
%  \caption{Two types of congestion between tenants}
%  %\label{fig1}
%\end{figure}

\subsection{Tenants-counter}
With the rapid development of the programmable switch in recent years, despite the WFQ that cannot be achieved we mentioned above, there are still many usable and excellent features. If we absolutely deny the usage in the bandwidth allocation works, is obvious unwise. Therefore, we develop an additional design called Tenants-counter, using the programmable switch to improve the performance of ProNet. 

 
The reason why our system implies Tenants-counter is in the development of ProNet, we have observed a problem. Only with the control on the host end the system can be aware of the congestion situation by the ECN signal from flows of different tenants but the system can't detect which tenants' flows are the congested flow congesting with, not to mention the place of the congestion happens. Figure 4 shows two situations in which the host-ends will receive the same packets with the same ECN signal but only the rates of flows in Figure 4(a) need to be limited to the weighted fairness allocation speed because the congestion in the first figure happens between different tenants' flows. However, for the situation in Figure 4(b), the receiving end will receive the same tenants' packets with the ECN tag. In Figure 4(b), the two flows in link a are congested but they are flows from the same tenant, as well as link b. In this situation for some allocation strategies, the allocation between tenants A and B should may should not considered to be allocated in a weighted method due to they are not seizing one single link. Instead, those flows should be separated from the weighted allocated flows, just normally sent with an equal share between its own tenant's own-congested flows.


Although, the build-up price is still pretty high, and the queuing systems on it are still not precise and swift comparable with the host end, the programmable switch has been developing quickly in recent days and has many remarkable functions like sending packets proactively.
% That's the reason why the programmable switches are still not mass deployed for the bandwidth and inter-queuing in nowadays's data centers. 
So in this part of the design, we just simply use the register in the switch for the network situation record and the packet sending function for feedback.
Figure 5 shows another version of \sys~ with the programmable switch used. As the figure shows, what we do in the programmable switch is just add a \textit{Tenant register table}. When a packet (or flow) is passing through this switch, this table will register its tenant info. If another tenant's packet (or flow) passes this switch, a new entry will be added to the table. Then the programmable switch will send a feedback packet with all the tenants' info from the table, which stands for the tenant information of the instance traffic through this switch. (The table entry also has a time-out counter for the expired flow and tenants' info).

\begin{figure}[t]
  \centering
  \resizebox{\linewidth}{!}{
    \begin{subfigure}[t]{0.5\linewidth}
      \centering
      \resizebox{\textwidth}{!}{
        \includegraphics{figures/fig4(a).png}
      }
      \caption{Intra-tenant Congestion}
      \label{fig:testbed-topos:a}
    \end{subfigure}\hfil

    \begin{subfigure}[t]{0.5\linewidth}
      \centering
      \resizebox{\textwidth}{!}{
        \includegraphics{figures/fig4(b).png}
      }
      \caption{Inter-tenant Congestion}
      \label{fig:testbed-topos:b}
    \end{subfigure}\hfil

      }
  \caption{Two types of congestion between tenants}
  \label{fig:testbed-topos}
\end{figure}

For the host-end, we add a new structure called \textbf{Non-Competitive Pool}. At first, all unit-flows are set as Non-Competitive and all classified into this pool. For all the unit-flows in the pool, they will be sent limitless which means they will be sent as much as possible for the best effort. However, when the host-end receives feedback from a switch, that means some or more of the unit-flows are congested with other tenants' flows. In this case, the corresponding unit-flows will be moved from the pool for the weighted allocation. In this way, with a little cooperation of the programmable switches, we can not only achieve the inter-tenants weighted allocation but also can detect the intra-tenant congestion situation.

\begin{figure}
	\centering
	\setlength{\abovecaptionskip}{0 cm}
	\includegraphics[width=3.5in]{figures/fig5.png}
	\caption{System Structure with Additional Design}
\end{figure}

There come many advantages along with the implementation of this design. In the data center, the flows are many and varied, for many applications, for example, send many short and frequent requests in the form of short flows. These kinds of short flows take a small slice of the bandwidth usage and are usually hard to measure with normal length flows. In our system, we can assign flows with a length less than we think as a short flow into the Non-Competitive Pool, then these flows will be sent limitlessly for better performance. Also we find this mechanism is practical for the situation if some flows is required as a high-priority of some tenants, and to maintain the quality of these flows, they can be assigned to the Non-Competitive Pool as well for the preferential transmission. In addition, after our evaluation, Tenants-counter is not necessary to be append to every nodes with programmable switches. Instead, with the deploy on some major nodes like the possible bottlenecks in the network, the problem mentioned above can be solved approximately.

